Are Data Experts Buying into Differentially Private Synthetic Data? Gathering Community Perspectives

Data privacy is a core tenet of responsible computing, and in the United States, differential privacy (DP) is the dominant technical operationalization of privacy-preserving data analysis. With this study, we qualitatively examine one class of DP mechanisms: private data synthesizers. To that end, we conducted semi-structured interviews with data experts: academics and practitioners who regularly work with data. Broadly, our findings suggest that quantitative DP benchmarks must be grounded in practitioner needs, while communication challenges persist. Participants expressed a need for context-aware DP solutions, focusing on parity between research outcomes on real and synthetic data. Our analysis led to three recommendations: (1) improve existing insufficient sanitized benchmarks; successful DP implementations require well-documented, partner-vetted use cases, (2) organizations using DP synthetic data should publish discipline-specific standards of evidence, and (3) tiered data access models could allow researchers to gradually access sensitive data based on demonstrated competence with high-privacy, low-fidelity synthetic data.

==> bar_chart.tex <==
\newcommand{\tightspacing}{\renewcommand{\baselinestretch}{0.8}\normalsize}

\begin{figure*}
\begin{tikzpicture}

%% Percent of participants expressing... as a column header
\begin{axis}[
    xbar,
    width=5cm,
    height=8cm,
    y axis line style = { opacity = 0 },
    axis x line       = none,
    tickwidth         = 0pt,
    legend style={at={(1,1)}, anchor=north west},
    yticklabel style={execute at begin node=\tightspacing, align=right,text width=10cm, font=\footnotesize},
    ytick             = data,
    enlarge y limits  = 0.2,
    symbolic y coords = {
        \censusq,
        \syntheticq,
        \validationq,
        \skepticismq,
        \needq,
        \lawq,
    },
    nodes near coords={\pgfmathprintnumber\pgfplotspointmeta\%},
    nodes near coords align={horizontal},
    xtick={0,20,40,60,80,100},
    xticklabels={0\%,20\%,40\%,60\%,80\%,100\%},
]

\addplot[fill=highpp, bar width=0.2cm] coordinates {
    (64,\censusq)
    (73,\lawq) 
    (82,\needq)
    (82,\skepticismq) 
    (82,\validationq)
    (73,\syntheticq)
};

\addplot[fill=lowpp, bar width=0.2cm] coordinates {
    (0,\censusq)
    (80,\lawq) 
    (80,\needq)
    (100,\skepticismq) 
    (100,\validationq)
    (40,\syntheticq)
};

\addplot[fill=overall, bar width=0.2cm] coordinates {
    (43,\censusq)
    (75,\lawq) 
    (81,\needq)
    (88,\skepticismq) 
    (88,\validationq)
    (63,\syntheticq)
};

\legend{High PP, Low PP, Overall}

\end{axis}
\end{tikzpicture}
% \vspace{-1.2cm}
\caption{Percent of participants discussing general topics. Presented overall, as well as sorted by participants with above participant average privacy prior (``High PP'') and below participant average privacy prior (``Low PP'').}
\label{fig:percent}
\end{figure*}
